Destructive breakdown studies of irradiated LGADs at beam tests for the ATLAS HGTD

In the past years, it has been observed at several beam test campaigns that irradiated LGAD sensors break with a typical star shaped burn mark when operated at voltages much lower than those at which they were safely operated during laboratory tests. The study presented in this paper was designed to determine the safe operating voltage that these sensors can withstand. Many irradiated sensors from various producers were tested in two test beam facilities, DESY (Hamburg) and CERN-SPS (Geneva), as part of ATLAS High Granularity Timing Detector (HGTD) beam tests. The samples were placed in the beam and kept under bias over a long period of time in order to reach a high number of particles crossing each sensor. Both beam tests lead to a similar conclusion, that these destructive events begin to occur when the average electric field in the sensor becomes larger than 12 Volts per micrometre.

==> journal/Makefile <==
# Makefile for creating an ATLAS paper draft using journal classes

TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
DVIPS    = dvips
DVIPDF   = dvipdf
OPEN     = open

TEXFILES = $(wildcard *.tex)

.PHONY: texlive clean

all: atlas-jinst

texlive:
	for file in $(TEXFILES); do \
	  if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	    echo "Changing texlive value in $$file"; \
	    sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $$file; \
	  else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \
	done

atlas-elsevier: atlas-elsevier.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-jhep: atlas-jhep.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-jinst: atlas-jinst.pdf
	@echo "Made $<"
	$(OPEN) $<

atlas-revtex: atlas-revtex.pdf
	@echo "Made $<"
	# $(OPEN) $<

run_latex: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $< and $(basename $<).pdf"

# Standard LaTeX targets
%.pdf: %.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.dvi: $(BASENAME).tex
	$(LATEX)    $<
	$(LATEX)    $<

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf \
	 *.spl *-revtexNotes.bib *.run.xml *.synctex.gz *~

cleanall: clean
	-rm *.pdf

